Bridging the Gap between Decision and Logits in Decision-based Knowledge Distillation for Pre-trained Language Models

Conventional knowledge distillation (KD) methods require access to the internal information of teachers, e.g., logits. However, such information may not always be accessible for large pre-trained language models (PLMs). In this work, we focus on decision-based KD for PLMs, where only teacher decisions (i.e., top-1 labels) are accessible. Considering the information gap between logits and decisions, we propose a novel method to estimate logits from the decision distributions. Specifically, decision distributions can be both derived as a function of logits theoretically and estimated with test-time data augmentation empirically. By combining the theoretical and empirical estimations of the decision distributions together, the estimation of logits can be successfully reduced to a simple root-finding problem. Extensive experiments show that our method significantly outperforms strong baselines on both natural language understanding and machine reading comprehension datasets.

==> figs/ablation-mc-eps.tex <==
\begin{figure}[t]
\centering
\small
\subfloat{
  \begin{tikzpicture}
\begin{axis}[
    xlabel={Sampling time $N$},
    xmin=0,
    % xmode=log,
    ylabel={Accuracy}, ylabel near ticks,
    ymin=50, ymax=52,
    % log ticks with fixed point,
    % x tick label style={/pgf/number format/sci},
    % xtick={0,  20,   40, 60,   80, 100},
    ytick={50.0, 50.5, 51.0, 51.5, 52.0},
    y tick label style={
        /pgf/number format/.cd, fixed, fixed zerofill, precision=2, /tikz/.cd
    },
    ymajorgrids=true,
    grid style=dashed,
    width=\linewidth,height=0.6\linewidth,
    xtick pos=left,
    ytick pos=left,
    nodes near coords,
    every node near coord/.append style={font=\tiny,color=black,xshift=23pt,yshift=-2pt,anchor=east},
    coordinate style/.condition=
{\coordindex>=2}{xshift=-8pt,yshift=8pt},
    nodes near coords style={/pgf/number format/.cd,fixed,fixed zerofill,precision=2},
]

\addplot[
    color=MyDarkBlue,
    mark=o,
    ]
    coordinates {
    (1,50.15)
    (2,50.39)
    (5,50.46)
    (10,51.75)
    (20,51.77) % 暂时跑出两个随机种子，先放上
    (40,51.54) % 暂时跑出两个随机种子，先放上
    };
\end{axis}
\end{tikzpicture}
}
\vspace{-7pt}
\subfloat{\resizebox{\columnwidth}{!}{
\begin{tikzpicture}
\begin{semilogxaxis}[
    xlabel={Error bound $\epsilon$},
    ylabel={Accuracy}, ylabel near ticks,
    ymin=50.5, ymax=52,
    xmode=log,
    xtick={1e-4, 1e-3, 1e-2, 1e-1, 1},
    xticklabels={$10^{-4}$,$10^{-3}$,$10^{-2}$,$10^{-1}$,$1$},
    % log ticks with fixed point,
    % x tick label style={/pgf/number format/sci},
    % xtick={0,  20,   40, 60,   80, 100},
    ytick={50.5, 50.75, 51.00, 51.25, 51.50, 51.75, 52.00},
    y tick label style={
        /pgf/number format/.cd, fixed, fixed zerofill, precision=2, /tikz/.cd
    },
    ymajorgrids=true,
    grid style=dashed,
    width=\linewidth,height=0.6\linewidth,
    xtick pos=left,
    ytick pos=left,
    nodes near coords,
    every node near coord/.append style={font=\tiny,color=black},
    nodes near coords style={/pgf/number format/.cd,fixed,fixed zerofill,precision=2}
]

\addplot[
    color=MyDarkBlue,
    mark=o,
    ]
    coordinates {
    (1,50.74)
    (1e-1,51.69)
    (1e-2,51.71)
    (1e-3,51.75)
    (1e-4,51.82)
    };
\end{semilogxaxis}
\end{tikzpicture}
}
}
\caption{Comparison of different error bounds $\epsilon$ of teacher logits estimation in the theoretical derivation step (top), and sampling time $N$ of test-time data augmentation in the empirical estimation step (bottom). Averaged results over 5 different random seeds on the dev set of RACE-High are reported.}
\label{fig:ablation-mc-eps}
\end{figure}

==> tables/MRC-main.tex <==
\begin{table*}[htpb]
    \centering
    \small % lipeng
    \begin{tabular}{l|ccc|c|ccc|c|ccc|c}
        \toprule
        \multirow{2}{*}{Methods} & \multicolumn{3}{c|}{RACE} & \multirow{2}{*}{DREAM} & \multicolumn{3}{c|}{RACE} & \multirow{2}{*}{DREAM} & \multicolumn{3}{c|}{RACE} & \multirow{2}{*}{DREAM}
        \\
        \cmidrule{2-4}
        \cmidrule{6-8}
        \cmidrule{10-12}
        & Middle & High & All &
        & Middle & High & All &
        & Middle & High & All & \\
        \midrule
        % Architecture & \multicolumn{2}{c}{Teacher BERT$_{\rm BASE}$}
        % \\
        % \midrule
        Teacher & 68.25 & 61.21 & 66.74 & 61.39 &
                        &       & 69.94 &       &
                  68.25 & 61.21 & 66.74 & 61.39 \\
        \midrule
        Student & 51.03 & 47.25 & 49.94 & 50.98 &
                  51.03 & 47.25 & 49.94 & 50.98 &
                  59.11 &       &       &       \\
        \midrule
        Standard KD & 54.12 & 48.95 & 53.08 & 52.33 &
                            &       &       &       &
                            &       &       &       \\
        \midrule
        Hard $\star$ & 51.60 & \underline{47.93} & 50.29 & 49.83 &
                             &       &       &       &
                       59.64 &       &       &       \\
        Noisy Logits $\star$ & 50.57 & 46.30 & 49.86 &
                             & 50.57 & 46.30 & 49.86 &
                             &       & 51.12 &       \\
        Smooth $\star$ & \underline{51.71} & 46.93 & 49.56 & \underline{51.48} &
                                           &       &       &       &
                                    59.68  &       &       &       \\
        Surrogate & 51.28 & 47.90 & \underline{51.03} & 51.25 &
                    51.28 & 47.90 & 51.03 & 51.25 &
                          &       &       &       \\
        \rowcolor{Gray}
        \DBKD $\star$ & \textbf{52.81} & \textbf{48.89} & \textbf{52.17} & \textbf{51.85} &
                                       &       &       &       &
                                61.10 &       &   58.01  &       \\
        \bottomrule
    \end{tabular}
    \caption{Results on the test set of RACE and DREAM dataset. We bold the \textbf{best} scores and highlight the \underline{second best} scores. We use BERT$_{\rm BASE}$ as the teacher architecture and 4-layer BERT model as the student architecture. The best results except \textbf{Teacher} and \textbf{Standard KD} have been bolded. Decision-based methods are marked with $\star$ in the tables, and our method is marked with gray background for easy reference.}
    \label{tab:mrc-main}
\end{table*}


==> tables/ablation.tex <==
\begin{table}
    \centering
    \small % lipeng
    \begin{tabular}{l|c}
        \toprule
        Methods & RACE-High \\
        \midrule
        \DBKD & 51.75 \\
        \quad w/o Emperical Estimation & {\color{red}TODO} \\
        \quad w/o Theoretical Derivation & 51.64 \\
        \bottomrule
    \end{tabular}
    \caption{Ablation studies for the emperical estimation step (Section~\ref{sec:method-detail}) and the theoretical derivation step (Section~\ref{sec:recon}) on the dev set of RACE-High.\qh{TODO: 1 result left, by 1.18}}. 
    \label{tab:ablation}
\end{table}


==> tables/race-6l.tex <==
\begin{table}
    \centering
    \small % lipeng
    \begin{tabular}{l|ccc}
        \toprule
        Methods & \ Middle & High & All \\
        \midrule
        Teacher & 68.66 & 62.56 & 67.79 \\
        \midrule
        Student & 60.53 & 53.71 & 58.16 \\
        \midrule
        Standard KD & 62.52 & 56.78 & 60.98 \\
        \midrule
        Noisy Logits $\star$ & 60.46 & 53.03 & -- \\
        Smooth $\star$ & 60.65 & 53.59 & -- \\
        Hard $\star$ & 60.64 & 53.90 & -- \\
        Surrogate & 60.70 & 53.31 & -- \\
        \rowcolor{Gray}
        \DBKD $\star$ & \textbf{61.84} & \textbf{55.66} & \textbf{59.97} \\
        \bottomrule
    \end{tabular}
    \caption{Results of BERT$_{\rm BASE}$ teacher models and 6-layer student models on the validation set of RACE dataset.\qh{TODO test results}}. 
    \label{tab:race-6l}
\end{table}


==> tables/race-large.tex <==
\begin{table}
    \centering
    \small % lipeng
    \begin{tabular}{l|ccc}
        \toprule
        Methods & \ Middle & High & All \\
        \midrule
        Teacher & 72.35 & -- & -- \\
        \midrule
        Student & 50.52 & 49.70 & 51.25 \\
        \midrule
        Standard KD & -- & -- & -- \\
        \midrule
        Noisy Logits $\star$ & 50.18 & 49.30 & 51.37 \\
        Smooth $\star$ & -- & -- & -- \\
        Hard $\star$ & -- & -- & -- \\
        Surrogate & 50.46 & 50.33 & 52.68 \\
        \rowcolor{Gray}
        \DBKD $\star$ & -- & -- & -- \\
        \bottomrule
    \end{tabular}
    \caption{Results of BERT$_{\rm LARGE}$ teacher models and 4-layer student models on the validation set of RACE dataset.\qh{TODO test results}}. 
    \label{tab:race-large}
\end{table}


==> tables/race-main-old.tex <==
\begin{table}
    \centering
    \small % lipeng
    \begin{tabular}{l|ccc|c}
        \toprule
        \multirow{2}{*}{Methods} & \multicolumn{3}{c|}{RACE} & \multirow{2}{*}{DREAM} \\
        \cmidrule{2-4}
        & Middle & High & All & \\
        \midrule
        Teacher & 68.25 & 61.21 & 66.74 & 61.39 \\
        \midrule
        Student & 51.03 & 47.25 & 49.94 & 50.98 \\
        \midrule
        Standard KD & 54.12 & 48.95 & 53.08 & 52.33 \\
        \midrule
        Hard $\star$ & 51.60 & \underline{47.93} & 50.29 & 49.83 \\
        Noisy Logits $\star$ & 50.57 & 46.30 &49.86 &  \\
        Smooth $\star$ & \underline{51.71} & 46.93 & 49.56 & \underline{51.48} \\
        Surrogate & 51.28 & 47.90 & \underline{51.03} & 51.25 \\
        \rowcolor{Gray}
        \DBKD $\star$ & \textbf{52.81} & \textbf{48.89} & \textbf{52.17} & \textbf{51.85} \\
        \bottomrule
    \end{tabular}
    \caption{Results on the test set of RACE and DREAM dataset. We bold the \textbf{best} scores and highlight the \underline{second best} scores. We use BERT$_{\rm BASE}$ as the teacher architecture and 4-layer BERT model as the student architecture. The best results except \textbf{Teacher} and \textbf{Standard KD} have been bolded. Decision-based methods are marked with $\star$ in the tables, and our method is marked with gray background for easy reference.}
    \label{tab:race-main}
\end{table}


==> tables/teaser.tex <==
\begin{table}[t]
    \small % lipeng
    \centering
    \begin{tabular}{l|c|c}
         \toprule
         Method  & \makecell{Teacher\\knowledge} & KD target \\
         \midrule
         \makecell[l]{Standard KD\\\cite{hintonkd}} & logits & soft label \\
         \midrule
         \makecell[l]{QEKD\\\cite{qekd}} & decision & hard label \\
         \midrule
         \makecell[l]{DFMS-HL\\\cite{hardstealing}} & decision & hard label \\
         \midrule
         \makecell[l]{DB3KD\\\cite{wang2021dbkd}} & decision & soft label \\
         \midrule
         \DBKD & decision & soft label \\
         \bottomrule
    \end{tabular}
    \caption{A brief overview of standard KD and decision-based KD methods. Both QEKD and DFMS-HL train student model on the hard label of teacher prediction. Although DB3KD constructs soft label, it is infeasible for discrete text inputs. Our \DBKD method \qh{...}}
    \label{tab:teaser}
\end{table}
